Byzantine Fault-Tolerant Min-Max Optimization

In this paper, we consider a min-max optimization problem under adversarial manipulation, where there are $n$ cost functions, up to $f$ of which may be replaced by arbitrary faulty functions by an adversary. The goal is to minimize the maximum cost over $x$ among the $n$ functions despite the faulty functions. The problem formulation could naturally extend to Byzantine fault-tolerant distributed min-max optimization. We present a simple algorithm for Byzantine min-max optimization, and provide bounds on the output of the algorithm. We also present an approximate algorithm for this problem. We then extend the problem to a distributed setting and present a distributed algorithm. To the best of our knowledge, we are the first to consider this problem.

==> algo-2.tex <==

\section{Fault-tolerant algorithm \#2}

In this section, we make two assumptions:
(i) We assume that the cost functions are non-negative. (ii)
We assume a constrained version of the problem, with argument $x$ constrained to a hyperrectangle $X$.

Recall that
\begin{align}
    h_{f}(x) = \underset{i\in[n]}{\mathrm{rank}_{f+1}}(Q_i(x))
\end{align}
Let us also define
\begin{eqnarray}
g_1(x) & = &\underset{i\in\H}{\mathrm{rank}_1}(Q_i(x)) \\
    g_{f}(x)& = & \underset{i\in\H}{\mathrm{rank}_{f+1}}(Q_i(x))
\end{eqnarray}
Then, 
$$g_f(x)\leq h_f(x)\leq g_1(x).$$

Let us assume that the cost function $Q_i(x)$ of any non-faulty agent $i$ is Lipschitz continuous with Lipschitz constant $L$ in $X$. Then,

$$|Q_i(x_1)-Q_i(x_2)| \leq L \|x_1-x_2\|, ~~~~ i\in\H$$

Note that we do not make any assumptions about the
faulty functions (i.e., $j\not\in\H$). 

We now show a claim to be used later.

\begin{claim}
\label{claim:Lipschitz}
Given that function $Q_i(x)$ for non-faulty agent $i$ is Lipschitz continuous with parameter $L$ in $X$, $g_1(x)$ is also Lipschitz continuous with parameter $L$.
\end{claim}
\begin{proof}
Consider any two points $x_1,x_2\in X$. Without loss of generality, suppose that
$$g_1(x_1)\geq g_1(x_2).$$
Recall that $$g_1(x) = \underset{i\in\H}{\mathrm{rank}_1}(Q_i(x)).$$
Let
$$q = \arg\max_{i\in\H} Q_i(x_1)$$
and
$$r = \arg\max_{i\in\H} Q_i(x_2)$$
Then, $g_1(x_1)=Q_q(x_1)$ and $g_1(x_2)=Q_r(x_2)$.

Now,
$Q_q(x_2)\leq Q_r(x_2)$ because of the definition of $r$.
\begin{eqnarray*}
g_1(x_1) - g_1(x_2) & = & Q_q(x_1) - Q_r(x_2) \\
& \leq & Q_q(x_1) - Q_q(x_2)  \mbox{~~~~because $Q_q(x_2)\leq Q_r(x_2)$}\\
& \leq & L \|x_1-x_2\| \mbox{~~~~because $Q_q(x)$ is Lipschitz with parameter $L$}
\end{eqnarray*}
Also, $g_1(x_1) - g_1(x_2)\geq 0$.
Thus, we have that
$$|g_1(x_1)-g_1(x_2)|\leq L \|x_1-x_2\|$$
proving that $g_1(x)$ is Lipschitz continuous with parameter $L$.

\end{proof}

Recall that, for convenience, we have assumed that the constraint set $X$ is a hyperrectangle.
Now we consider the following algorithm: 
\begin{itemize}
    \item Partition $X$ into hyperrectangles $S_j$ with $C_j$ denoting the center of $S_j$ and $d_j$ denoting the diameter of $S_j$ such that, for a specified constant parameter $\epsilon$,
    \begin{align}
    L d_j < \epsilon\,\min_i h_f(C_i) \label{eq_d}
\end{align}
where the minimum is over all the hyperrectangles in the subdivision of $X$.
\item Let $k=\arg\min_i h_f(C_i)$. Let $\overline{x}=C_k$. Output $\overline{x}$.
\end{itemize}
The DIRECT algorithm \cite{direct} results in a subdivision that is similar to that performed by the above algorithm.

Now,
\begin{eqnarray}
g_f(\overline{x}) & \leq & h_f(\overline{x}) 
\label{e_g_f}
\end{eqnarray}
and
\begin{eqnarray}
h_f(\overline{x})
& = & h_f(C_k)  \nonumber \\ \nonumber
& \leq & h_f(C_j) ~~~~\forall j \mbox{~~~~due to definition of $C_k$} \\ \nonumber
& \leq & g_1(C_j) ~~~~\forall j \mbox{~~~~due to definition of $h_f$ and $g_1$} \\ \nonumber
& \leq & \min_{x\in S_j} g_1(x) + Ld_j ~~~~\forall j
\mbox{~~~~due to Claim \ref{claim:Lipschitz}}\\ \nonumber
& \leq & \min_{x\in S_j} g_1(x) + \epsilon \, h_f(\overline{x}) 
~~~~\forall j \mbox{~~~~due to the above algorithm} \\ \nonumber
\Rightarrow h_f(\overline{x}) & \leq & \min_{x\in X} g_1(x) + \epsilon\,h_f(\overline{x}) 
~~~~\mbox{because $\cup_j S_j=X$} \\
\Rightarrow
h_f(\overline{x}) & \leq & \left(\frac{1}{1-\epsilon}\right) \, \min_{x\in X} g_1(x) \label{e_h_f}
\end{eqnarray}
Equations \eqref{e_g_f} and \eqref{e_h_f} imply that
$$g_f(\overline{x}) \leq \left(\frac{1}{1-\epsilon}\right) \, \min_{x\in X} g_1(x)$$
This implies that at least $|\H|-f$ of the non-faulty cost functions are upper bounded by
$$\left(\frac{1}{1-\epsilon}\right) \, \min_{x\in X} g_1(x)$$
at the output $\overline{x}$ of the algorithm presented earlier in this section.
On the other hand, Claim \ref{claim:1} indicates that
$$g_f(\widehat{x}) \leq \min_{x\in X} g_1(x).$$
Thus, the algorithm in this section results in
an increase in the upper bound by a factor of $\frac{1}{1-\epsilon}$.
As a trade-off, the algorithm in this section does not look for the exact global minimum of $h_f(x)$, and instead only approximates the minimum. The algorithm in Section \ref{sec:algo_1} finds the exact minimum $\widehat{x}$ of $h_f(x)$.




    

==> redundancy.tex <==

    \section{TODO}

    \begin{itemize}
        \item Sufficiency condition: $\min g_1 = \min g_{2f+1}$, also necessity condition (photo)
        \item \sout{Correctness of direct with faults $\rightarrow$ it wouldn't divide the same square all the time}
        \item Can we bound the convergence rate DIRECT with faults?
        
        e.g.: assume $h_1/h_{f+1}= R$ can we claim it would take no less than $R$ iterations to divide...
    \end{itemize}

    \section{\textcolor{blue}{existing comments}}

    \begin{itemize}
        \item At the beginning of Section 3 (need discussion)
        \item At the end of Section 3 (need discussion)
        \item Before the last two paragraphs in the proof of Claim~\ref{claim:min-max-everywhere-dense}.
    \end{itemize}

\section{Redundancy condition and its necessity and sufficiency}
The following results do not assume the convexity of cost functions.

\begin{definition}[$f$-resilience]
    A deterministic distributed min-max optimization algorithm is said to be $f$-resilient, if it outputs a minimum value of min-max optimization problems distributively, in the presence of up to $f$ Byzantine faulty agents.
\end{definition}
\begin{definition}[$2f$-redundancy]
    A group of cost functions is said to be $2f$-redundant, if there are at least $2f+1$ agents that have the same minimum value, and their minimum sets have at least one common point.
\end{definition}
\begin{lemma}
    Suppose $k$ cost functions $Q_1,...,Q_k$ have the same minimum value $v^*$, and their minimum sets have at least one minimum point $x^*$, then $h_1(x)=\underset{i\in[k]}{\mathrm{rank}_1}Q_i(x)$ also minimize at that point and has the same minimum value.
    \label{lemma:largest-minimum-value}
\end{lemma}
\begin{proof}
    By the definition of $h_1(x)$, $h_1(x)$ at $x^*$ is $v^*$, since all $Q_i(x)$'s have $v^*=Q_i(x^*)$.

    Suppose $h_1(x)$ minimizes at some other point $x'$, and any common minimum point $x^*$ of all $Q_i$'s is not $h_1(x)$'s minimzer. It follows that $h_1(x')\leq v^*$. That is, there exists a $j\in[k]$, $Q_j(x')\leq v^*$. Also, for all $i\in[k]$, $Q_i(x')\leq Q_j(x')$. 
    There are 2 cases: 
    \begin{enumerate}[label=\roman*)]
        \item If $Q_j(x')<v^*$, it indicates that $Q_j(x')<Q_j(x^*)=\min Q_j(x)$, which is contradictory to the meaning of minimum.
        \item If $Q_j(x')=v^*$, it follows that for all $i\in[k]$, $Q_i(x')\leq Q_j(x')=v^*$. Since $v^*=\min Q_i(x)$ for all $i$, it must be that $Q_i(x')=v^*$ for all $i$ as well. Therefore, $x'$ is also a common minimum point of all $k$ cost functions, which is contradictory to the definition of $x'$.
    \end{enumerate}
    Hence, the proof.
\end{proof}
\begin{claim}[Sufficiency]
    A $f$-resilient distributed min-max optimization algorithm exists, if the cost functions satisfy $2f$-redundancy.
\end{claim}
\begin{proof}
    We show this constructively. Consider the following algorithm:
    \begin{itemize}
        \item[\textbf{Step 1}] The server collects cost functions of all agents. Each non-faulty agent $i$ sends its actual cost function, denoting it as $Q_i(x)$. Each faulty agent $j$ may send an arbitrary function, denoting it as $Q_j(x)$.
        \item[\textbf{Step 2}] The server calculates the minimum value $v_i$ of each $Q_i(x)$.
        \item[\textbf{Step 3}] The server outputs the $f+1$ largest $v_i$ (breaking ties by $i$ in ascending order).
    \end{itemize}
    Suppose $2f$-redundancy is satisfied. With up to $f$ faulty agents, there are three possible cases:
    \begin{itemize}
        \item[\textbf{Case 1}] The largest minimum value $v_i$ among faulty agents is the largest $\leq f$ among all agents. The $f+1$ largest minimum value among all agents is the largest minimum value of non-faulty agents.
        \item[\textbf{Case 2}] The largest minimum value $v_i$ among faulty agents is the $f+1$-largest among all agents. It follows that $v_i$ must be equal to the largest minimum value of non-faulty agents.
        \item[\textbf{Case 3}] The largest minimum value $v_i$ among faulty agents is at most $f+2$-largest among all agents. The $f+1$ largest minimum value among all agents is the largest minimum value of non-faulty agents.
    \end{itemize}
    In all three cases, by outputting the $f+1$ largest $v_i$, the algorithm outputs the largest minimum value of non-faulty agents. By $2f$-redundancy and  Lemma~\ref{lemma:largest-minimum-value}, such value is also the minimum value of $h_1(x)$. Therefore, the algorithm is $f$-resilient.
\end{proof}
\begin{claim}[Necessity]
    A $f$-resilient distributed min-max optimization algorithm exists, only if $2f$-redundancy is satisfied.
\end{claim}
\begin{proof}
    Suppose there is a deterministic $f$-resilient distributed min-max optimization algorithm. 
\end{proof}
